AI Content Self-Detection for Transformer-based Large Language Models

$ $The usage of generative artificial intelligence (AI) tools based on large language models, including ChatGPT, Bard, and Claude, for text generation has many exciting applications with the potential for phenomenal productivity gains. One issue is authorship attribution when using AI tools. This is especially important in an academic setting where the inappropriate use of generative AI tools may hinder student learning or stifle research by creating a large amount of automatically generated derivative work. Existing plagiarism detection systems can trace the source of submitted text but are not yet equipped with methods to accurately detect AI-generated text. This paper introduces the idea of direct origin detection and evaluates whether generative AI systems can recognize their output and distinguish it from human-written texts. We argue why current transformer-based models may be able to self-detect their own generated text and perform a small empirical study using zero-shot learning to investigate if that is the case. Results reveal varying capabilities of AI systems to identify their generated text. Google's Bard model exhibits the largest capability of self-detection with an accuracy of 94\%, followed by OpenAI's ChatGPT with 83\%. On the other hand, Anthropic's Claude model seems to be not able to self-detect.

==> Flowcharts/methodology.tex <==
\begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop] {Utilizing a Dataset of Topics};
        \node (prompts) [process, below of=dataset] {Provide Identical Prompts};
        \node (generate) [process, below of=prompts] {Essay Generation (250 words) by Each AI};
        \node (compile) [startstop, below of=generate] {Compile Essays into Dataset};
        
        % Arrows
        \draw [arrow] (dataset) -- (prompts);
        \draw [arrow] (prompts) -- (generate);
        \draw [arrow] (generate) -- (compile);
        
        \end{tikzpicture}

        \caption{Dataset Preparation}

    \end{figure*}

    \vspace{1cm}

    \begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.4, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Original Text};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {AI Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {YES} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {NO}(no);
        
        \end{tikzpicture}
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.4, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Paraphrased Text};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {AI Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {YES} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {NO}(no);
        
        \end{tikzpicture}
        

        \caption{AI System's Self-identification Workflow}

    \end{figure*}

    \vspace{1cm}
    
    \begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.6, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Original Text};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {ZeroGPT Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {YES} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {NO}(no);
        
        \end{tikzpicture}
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.6, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Paraphrased Text};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {ZeroGPT Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {YES} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {NO}(no);
        
        \end{tikzpicture}
        \caption{ZeroGPT Plagiarism Check Workflow}

    \end{figure*}

    \newpage

    \begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.6, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Human-written Text};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {AI Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {Verdict from AI} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {Verdict from AI} (no);
        
        \end{tikzpicture}
        \caption{Human Text Identification Workflow}

    \end{figure*}

    \vspace{1cm}
    
    \begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.6, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {AI-generated Text*};
        \node (decision) [decision, below of=dataset, yshift=-0.75cm] {AI Identification};
        \node (yes) [process, below of=decision, xshift=-2.5cm] {Record "TRUE"};
        \node (no) [process, below of=decision, xshift=2.5cm] {Record "FALSE"};
        
        % Arrows
        \draw [arrow] (dataset) -- (decision);
        \draw [arrow] (decision) -| node[anchor=east] {Verdict from AI} (yes);
        \draw [arrow] (decision) -| node[anchor=west] {Verdict from AI} (no);
        
        \end{tikzpicture}
        \caption{AI-generated Text Identification Workflow}

    \end{figure*}

    \vspace{1cm}

    \begin{figure*}[!hbt]
        \centering
        \begin{tikzpicture}[node distance=1.5cm, auto]

        % Define block styles
        \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!20]
        \tikzstyle{decision} = [diamond, minimum width=3cm, aspect=1.6, minimum height=1cm, text centered, draw=black, fill=gray!30]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        
        % Nodes
        \node (dataset) [startstop, process] {Human-written or AI-generated Text};
        \node (result) [process, below of=dataset, yshift=-0.25cm] {AI Identification};
        \node (comparison) [decision, below of=result, yshift=-1.0cm] {Result Comparison};
        \node (yes) [process, below of=comparison, xshift=-2.5cm] {Record "CORRECT"};
        \node (no) [process, below of=comparison, xshift=2.5cm] {Record "INCORRECT"};
        
        % Arrows
        \draw [arrow] (dataset) -- (result);
        \draw [arrow] (result) -- node[anchor=west] {Verdict from AI} (comparison);
        \draw [arrow] (comparison) -| node[anchor=east] {Correct Identification} (yes);
        \draw [arrow] (comparison) -| node[anchor=west] {Incorrect Identification} (no);
        
        \end{tikzpicture}
        \caption{Mixed Text Identification Workflow}

    \end{figure*}

    
    \vspace{1cm}
    
    \textit{* Generated texts from other AI systems}

==> Tables/AI_Human_Identification.tex <==
\begin{table*}[!h]
        \centering
        \begin{tabular}{|c|c|}
            \hline 
            Model  &  Human Written Text Identification\\
            \hline
            ChatGPT & 76.00\% \\
            \hline
            BARD & 92.00\% \\
            \hline
            Claude & 84.00\% \\
            \hline
        \end{tabular}
        \caption{AI Systems' Human Text Identification Accuracy}
        \label{tab:table02}
    \end{table*}

==> Tables/AI_Self_Identification.tex <==
\begin{table*}[!h]
        \centering
        \begin{tabular}{|c|c|c|c|c|c|}
            \hline
            Model & \multicolumn{1}{|p{3cm}|}{\centering Detected \\ Generated \\ Text (Own)} & \multicolumn{1}{|p{3cm}|}{\centering Detected\\  Generated \& Paraphrased\\ Text (Own)} & \multicolumn{1}{|p{3cm}|}{\centering  Detected by\\ ZeroGPT  \\(Only Generated Text)} & \multicolumn{1}{|p{3cm}|}{\centering  Detected by\\  ZeroGPT\\(Generated \& Paraphrased Text)}
            \\
            \hline
            ChatGPT & 90.00\% & 40.00\% & 64.00\% & 32.00\%\\
            \hline
            BARD & 96.00\% & 92.00\% & 88.00\% & 76.00\%\\
            \hline
            Claude & 24.00\% & 80.00\% & 12.00\% & 8.00\%\\
            \hline
        \end{tabular}
        \caption{AI Systems' Self-identification Accuracy}
        \label{tab:table01}
    \end{table*}

==> Tables/Inter-AI_comparison.tex <==
\begin{table*}[!h]
        \centering
        \begin{tabular}{|c|c|c|c|}
            \hline 
              &  ChatGPT & Claude & BARD\\
            \hline
            ChatGPT & 90.00\%	& 60.00\%	& 50.00\%\\
            \hline
            Claude	& 10.00\%	& 24.00\%	& 40.00\%\\
            \hline
            BARD &	5.00\% &	0.00\% &	96.00\%\\
            \hline
        \end{tabular}
        \caption{AI Content Detection Comparison Among Inter AI-Systems}
        \label{tab:inter-ai}
    \end{table*}

==> Tables/Mixed_Comparison.tex <==
\begin{table*}[!hbt]
        \centering
        \begin{tabular}{|c|c|}
            \hline 
            Model  &  Human-AI Mixed Text Identification\\
            \hline
            ChatGPT & 46.00\% \\
            \hline
            BARD & 20.00\% \\
            \hline
            Claude & 56.00\% \\
            \hline
        \end{tabular}
        \caption{AI Systems' Mixed Text Identification Accuracy}
        \label{tab:table04}
    \end{table*}

==> Tables/accuracy_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|c|c|}
\hline
Subject & Accuracy & 95\% CI \\
\hline
Accuracy of 50 C ChatGPT generated vs 50 Human & 0.83 & 0.7564, 0.9036 \\
\hline
Accuracy of 50 ChatGPT Paraphrased vs 50 Human & 0.58 & 0.4833, 0.6767 \\
\hline
Accuracy of 50 BARD generated vs 50 Human & 0.95 & 0.9073, 0.9927 \\
\hline
Accuracy of 50 BARD Paraphrased vs 50 Human & 0.92 & 0.8668, 0.9732 \\
\hline
Accuracy of 50 Claude generated vs 50 Human & 0.54 & 0.4423, 0.6377 \\
\hline
Accuracy of 50 Claude Paraphrased vs 50 Human & 0.52 & 0.4221, 0.6179 \\
\hline
\end{tabular}
\caption{Accuracy Results}
\label{tab:supp_accuracy}
\end{table}

